Model Architecture Adaption for Bayesian Neural Networks

Bayesian Neural Networks (BNNs) offer a mathematically grounded framework to quantify the uncertainty of model predictions but come with a prohibitive computation cost for both training and inference. In this work, we show a novel network architecture search (NAS) that optimizes BNNs for both accuracy and uncertainty while having a reduced inference latency. Different from canonical NAS that optimizes solely for in-distribution likelihood, the proposed scheme searches for the uncertainty performance using both in- and out-of-distribution data. Our method is able to search for the correct placement of Bayesian layer(s) in a network. In our experiments, the searched models show comparable uncertainty quantification ability and accuracy compared to the state-of-the-art (deep ensemble). In addition, the searched models use only a fraction of the runtime compared to many popular BNN baselines, reducing the inference runtime cost by $2.98 \times$ and $2.92 \times$ respectively on the CIFAR10 dataset when compared to MCDropout and deep ensemble.

==> tables/stroke.tex <==
\begin{table*}[ht!]
    \caption{
        Results of Stroke prediction.
        % The objective is to predict the presence of heart disease in the patient.
    }
    \label{tab:heart}
    \begin{center}
    % \adjustbox{scale=0.8}{%        
    \begin{tabular}{c|ccccc}
    \toprule
    \multirow{1}*{Method}   
    & F1 Score    &AUROC & Accuracy & Certainty & NLL  \\
    \midrule
    & \multicolumn{5}{c}{In distribution data} \\
    \midrule
    Non-Bayesian	&$0.7048 \pm 0.0431$	&$0.8387 \pm 0.0403$	&$0.9772 \pm 0.0080$	&$0.9806 \pm 0.0015$	&$0.0839 \pm 0.0310$\\
    LRT	&$0.0000 \pm 0.0000$	&$0.5000 \pm 0.0000$	&$0.9504 \pm 0.0104$	&$0.9525 \pm 0.0021$	&$0.1608 \pm 0.0229$\\
    MCDropout	&$0.7149 \pm 0.0512$	&$0.8342 \pm 0.0309$	&$0.9726 \pm 0.0089$	&$0.9721 \pm 0.0057$	&$0.1156 \pm 0.0189$\\
    Ensemble	&$0.0000 \pm 0.0000$	&$0.5000 \pm 0.0000$	&$0.9400 \pm 0.0033$	&$0.9484 \pm 0.0007$	&$0.1640 \pm 0.0039$\\
    \midrule
    & \multicolumn{5}{c}{Out of distribution data} \\
    \midrule
    MAP	&$0.4246 \pm 0.1556$	&$0.5013 \pm 0.0078$	&$0.5022 \pm 0.0192$	&$0.8677 \pm 0.0361$	&$1.7713 \pm 0.8084$\\
    LRT	&$0.0000 \pm 0.0000$	&$0.5000 \pm 0.0000$	&$0.5168 \pm 0.0000$	&$0.8330 \pm 0.0007$	&$1.3841 \pm 0.0064$\\
    MCDropout	&$0.5025 \pm 0.1260$	&$0.5082 \pm 0.0055$	&$0.5065 \pm 0.0107$	&$0.8750 \pm 0.0356$	&$1.4933 \pm 0.3017$\\
    Ensemble	&$0.0000 \pm 0.0000$	&$0.5000 \pm 0.0000$	&$0.5168 \pm 0.0000$	&$0.8850 \pm 0.0091$	&$1.1974 \pm 0.0637$\\
    \bottomrule
    \end{tabular}
    % }
    \end{center}
\end{table*}
